Out-of-Order Sliding-Window Aggregation with Efficient Bulk Evictions and Insertions (Extended Version)

Sliding-window aggregation is a foundational stream processing primitive that efficiently summarizes recent data. The state-of-the-art algorithms for sliding-window aggregation are highly efficient when stream data items are evicted or inserted one at a time, even when some of the insertions occur out-of-order. However, real-world streams are often not only out-of-order but also burtsy, causing data items to be evicted or inserted in larger bulks. This paper introduces a new algorithm for sliding-window aggregation with bulk eviction and bulk insertion. For the special case of single insert and evict, our algorithm matches the theoretical complexity of the best previous out-of-order algorithms. For the case of bulk evict, our algorithm improves upon the theoretical complexity of the best previous algorithm for that case and also outperforms it in practice. For the case of bulk insert, there are no prior algorithms, and our algorithm improves upon the naive approach of emulating bulk insert with a loop over single inserts, both in theory and in practice. Overall, this paper makes high-performance algorithms for sliding window aggregation more broadly applicable by efficiently handling the ubiquitous cases of out-of-order data and bursts.

==> reviewresponse.tex <==
\pagenumbering{roman}

\section*{Response to Reviewer Comments}

{\large
Thank you for your thorough reviews!
All additions and modifications in the paper are highlighted in
\textcolor{blue}{blue}, with notes in the margins mapping them
to indiviual reviewer feedback.
Here is a summary of how we have addressed the revision requests~(RRs)
highlighted in the meta-review:\\

\begin{itemize}
  \item
    \textbf{Meta-Review RR1)} \textit{``Single node setup is assumed;
      partitioning to different nodes is not considered''.}\\
    \textbf{Response:}
      We have extended Section~\ref{sec:implementation} with a brief
      discussion of parallelism (such as SIMD on a single node and
      fission to potentially multiple nodes).

  \item
    \textbf{Meta-Review RR2)} \textit{``The algorithms are not
      implemented and tested in a real system''.}\\
    \textbf{Response:}
      To address this revision request, we re-implemented our
      algorithm in Java~(previously we only showed C++ results) and
      integrated it with Apache Flink~(the first representative for a
      real system mentioned by R3(D2)).
      We ran new experiments with that and report the results in the
      new Figure~\ref{fig:flink_bulkevict_geomean}.

  \item
    \textbf{Meta-Review RR3)} \textit{``The tested workloads are not
      realistic''.}\\
    \textbf{Response:}
      We ran new experiments pushing the window size to a new extreme
      of 1~billion entries and report the results in a new section,
      Section~\ref{sec:one_billion}.
      This is more than 238 times larger than the highest window size
      of 4,194,304 we used previously.

  \item
    \textbf{Meta-Review RR4)} \textit{``Limited novelty; the algorithm
      is an extension of FiBA with bulk insertions and evictions;
      there is missing related work on bulk inserts in B-trees for
      batch systems, and additional algorithms for sliding windows''.}\\
    \textbf{Response:}
      We have added the related work mentioned by reviewers to
      Section~\ref{sec:relatedwork}.
      Also, while we agree that the algorithm is an extension of FiBA
      with bulk insertions and evictions, in our opinion, this extension
      is both substantial and novel.

  \item
    \textbf{Meta-Review RR5)} \textit{``Experimental findings are not
      discussed adequately''.}\\
    \textbf{Response:}
      We ran new experiments for an ablation study and report the
      results in a new figure, Figure~\ref{fig:ablation}.
      Also, we made several other enhancements to the discussion in
      Section~\ref{sec:results}.
\end{itemize}

\vspace*{3mm}\noindent
Besides the above-mentioned revisions, we have also made many other
changes based on minor points raised in the reviews~(highlighted in
\textcolor{blue}{blue} like all our revisions).}

\newpage
\pagenumbering{arabic}

